Stronger Than You Think: Benchmarking Weak Supervision on Realistic Tasks

Weak supervision (WS) is a popular approach for label-efficient learning, leveraging diverse sources of noisy but inexpensive weak labels to automatically annotate training data. Despite its wide usage, WS and its practical value are challenging to benchmark due to the many knobs in its setup, including: data sources, labeling functions (LFs), aggregation techniques (called label models), and end model pipelines. Existing evaluation suites tend to be limited, focusing on particular components or specialized use cases. Moreover, they often involve simplistic benchmark tasks or de-facto LF sets that are suboptimally written, producing insights that may not generalize to real-world settings. We address these limitations by introducing a new benchmark, BOXWRENCH, designed to more accurately reflect real-world usages of WS. This benchmark features tasks with (1) higher class cardinality and imbalance, (2) notable domain expertise requirements, and (3) opportunities to re-use LFs across parallel multilingual corpora. For all tasks, LFs are written using a careful procedure aimed at mimicking real-world settings. In contrast to existing WS benchmarks, we show that supervised learning requires substantial amounts (1000+) of labeled examples to match WS in many settings.

==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    
    \answerYes{Yes, the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope.}
    
  \item Did you describe the limitations of your work?
    
    \answerYes{Yes, we describe this in \cref{limitations}.}
    
  \item Did you discuss any potential negative societal impacts of your work?
  
    \answerYes{Yes, we describe the potential negative and positive societal impacts of WS benchmarking in \cref{broader_impact}.}
    
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  
    \answerYes{We have carefully studied the ethics review guidelines and ensured all of the content in this paper conforms to them} 
    
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    
    \answerNA{}
    
	\item Did you include complete proofs of all theoretical results?
    
    \answerNA{}
    
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    
    \answerYes{We provide the codebase, dataset, and detailed instructions for running the code in \cref{sec:intro} and in the supplementary materials.}
    
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  
    \answerYes{We provide the training details in \cref{sec:experimental_setup}.}
    
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    
    \answerYes{All of our results and graphs include error bars, the error bar is set to be one standard deviation.}
    
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
 
    \answerYes{Yes, we include these details in \cref{sec:experimental_setup}.}
    
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  
    \answerYes{All of the existing assets used in this work are cited.}
    
  \item Did you mention the license of the assets?
    
    \answerYes{We discussed the license of all the assets in \cref{app:licenses}}
    
  \item Did you include any new assets either in the supplemental material or as a URL?
    
    \answerYes{We include all the new assets in the supplemental material. }
    
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    
    \answerYes{All of the data we are releasing are publicly available on online, and is mentioned in \cref{sec:data} and  \cref{app:licenses}}
  
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    
    \answerYes{All of the data we are releasing are doesn't contain personally identifiable information, and is mentioned in \cref{sec:data} }
    
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See \cref{sec:problem}, although we were the human participants. }
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See \cref{LF design pipeline}. We constructed LFs ourselves, i.e., we were the human subjects.}
\end{enumerate}

\end{enumerate}

==> sections/table.tex <==
\newpage
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|} \hline 
         &  Amazon31&  Banking77&  Claude9\\ \hline 
         6.25\% VS
CFT&  0.685,  0.685,  0.683,  0.682&  0.551, 0.551, 0.497, 0.497&  0.904, 0.904, 0.149, 0.874\\ \hline 
 Supervised Only& 0.660, 0.660, 0.659, 0.658& 0.234, 0.234, 0.167, 0.167&0.907, 0.907, 0.110, 0.864\\ \hline 
 12.5\% VS
CFT& 0.711, 0.711, 0.710, 0.709& 0.676, 0.676, 0.650, 0.650& 0.906, 0.906, 0.177, 0.877\\ \hline 
 Supervised Only& 0.701, 0.701, 0.702, 0.701& 0.378, 0.378, 0.318, 0.318&0.908, 0.908, 0.120, 0.866\\ \hline 
         25\% VS
CFT&  0.742, 0.742, 0.741, 0.740&  0.751, 0.751, 0.742, 0.742&  0.906, 0.906, 0.351, 0.895\\ \hline 
 Supervised Only& 0.736, 0.736, 0.736, 0.735& 0.567, 0.567, 0.530, 0.530&0.906, 0.906, 0.173, 0.870\\ \hline 
         50\% VS
CFT&  0.769, 0.769, 0.768, 0.767&  0.82, 0.82, 0.818, 0.818&  0.914, 0, 914, 0.493, 0.910\\ \hline 
 Supervised Only& 0.766, 0.766, 0.766, 0.765& 0.753, 0.753, 0.745, 0.745&0.911, 0.911, 0.256, 0.884\\ \hline 
         100\% VS
CFT&  0.791, 0.791, 0.791, 0.790&  0.866, 0.866, 0.865, 0.865&  0.914, 0.914, 0.558, 0.916\\ \hline 
 Supervised Only& 0.790, 0.790, 0.790, 0.789& 0.846, 0.846, 0.844, 0.844&0.913, 0.913, 0.349, 0.900\\ \hline
    \end{tabular}
    \caption{`accuracy',  `f1\_micro',  `f1\_macro',  `f1\_weighted' of the dataset with different validation size (VS).}
    \label{tab:my_label}
\end{table}




% \newpage

% \newpage
% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Label Function} & \textbf{Index} & \textbf{j} & \textbf{Polarity} & \textbf{Coverage} & \textbf{Overlaps} & \textbf{Conflicts} & \textbf{Correct} & \textbf{Incorrect} & \textbf{Emp. Acc.} & \textbf{Conflict Ratio} \\ \hline
% lf\_amino\_acid & 0 & 0 & 0.0187 & 0.0131 & 0.0124 & 16 & 14 & 0.5333 & 0.6667 \\ \hline
% lf\_replace & 1 & 0 & 0.0031 & 0.0019 & 0.0012 & 5 & 0 & 1 & 0.4 \\ \hline
% lf\_mutant & 2 &  & 0 & 0 & 0 & 0 & 0 & NaN & \\ \hline
% lf\_bind & 3 & 1 & 0.1095 & 0.0803 & 0.0697 & 104 & 72 & 0.5909 & 0.6364 \\ \hline
% lf\_interact & 4 & 1 & 0.0274 & 0.0174 & 0.0137 & 23 & 21 & 0.5227 & 0.5 \\ \hline
% lf\_affinity & 5 & 1 & 0.0523 & 0.0355 & 0.0286 & 63 & 21 & 0.75 & 0.5476 \\ \hline
% lf\_activate & 6 & 2 & 0.1195 & 0.0797 & 0.0728 & 66 & 126 & 0.3438 & 0.6094 \\ \hline
% lf\_increase & 7 & 2 & 0.1077 & 0.0734 & 0.0653 & 82 & 91 & 0.4740 & 0.6069 \\ \hline
% lf\_stimulate & 8 &  & 0 & 0 & 0 & 0 & 0 & NaN & \\ \hline
% lf\_upregulate & 9 & 2 & 0.0131 & 0.0093 & 0.0068 & 9 & 12 & 0.4286 & 0.5238 \\ \hline
% lf\_downregulate & 10 & 3 & 0.0168 & 0.0137 & 0.0081 & 19 & 8 & 0.7037 & 0.4815 \\ \hline
% lf\_reduce & 11 & 3 & 0.0604 & 0.0473 & 0.0373 & 55 & 42 & 0.5670 & 0.6186 \\ \hline
% lf\_inhibit & 12 & 3 & 0.3230 & 0.1711 & 0.1525 & 358 & 161 & 0.6898 & 0.4721 \\ \hline
% lf\_decrease & 13 & 3 & 0.0585 & 0.0436 & 0.0386 & 50 & 44 & 0.5319 & 0.6596 \\ \hline
% lf\_agonist & 14 & 4 & 0.0535 & 0.0411 & 0.0411 & 44 & 42 & 0.5116 & 0.7674 \\ \hline
% lf\_antagonist & 15 & 5 & 0.0803 & 0.0516 & 0.0516 & 75 & 54 & 0.5814 & 0.6434 \\ \hline
% lf\_combined\_modulator & 16 & 6 & 0.0062 & 0.0031 & 0.0031 & 2 & 8 & 0.2 & 0.5 \\ \hline
% lf\_allosteric & 17 & 6 & 0.0081 & 0.0081 & 0.0081 & 6 & 7 & 0.4615 & 1 \\ \hline
% lf\_cofactor & 18 & 7 & 0.0050 & 0.0037 & 0.0037 & 5 & 3 & 0.625 & 0.75 \\ \hline
% lf\_substrate & 19 & 8 & 0.0230 & 0.0174 & 0.0112 & 22 & 15 & 0.5946 & 0.4865 \\ \hline
% lf\_transport & 20 & 8 & 0.0436 & 0.0324 & 0.0274 & 29 & 41 & 0.4143 & 0.6286 \\ \hline
% lf\_catalyze & 21 & 8 & 0.0666 & 0.0386 & 0.0280 & 60 & 47 & 0.5607 & 0.4206 \\ \hline
% lf\_product & 22 & 8 & 0.0566 & 0.0404 & 0.0386 & 19 & 72 & 0.2088 & 0.6813 \\ \hline
% lf\_convert & 23 & 8 & 0.0137 & 0.0106 & 0.0062 & 12 & 10 & 0.5455 & 0.4545 \\ \hline
% lf\_not & 24 & 9 & 0.0274 & 0.0193 & 0.0193 & 23 & 21 & 0.5227 & 0.7045 \\ \hline
% \end{tabular}
% \caption{Current Accuracy for Each Label Function}
% \end{table}


% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Label Function} & \textbf{Index} & \textbf{j} & \textbf{Polarity} & \textbf{Coverage} & \textbf{Overlaps} & \textbf{Conflicts} & \textbf{Correct} & \textbf{Incorrect} & \textbf{Emp. Acc.} & \textbf{Conflict Ratio} \\ \hline
% lf\_amino\_acid & 0 & 0 & 0.0180 & 0.0143 & 0.0124 & 15 & 14 & 0.5172 & 0.6897 \\ \hline
% lf\_replace & 1 & 0 & 0.0031 & 0.0025 & 0.0006 & 5 & 0 & 1 & 0.2 \\ \hline
% lf\_mutant & 2 & 0 & 0.0317 & 0.0236 & 0.0205 & 13 & 38 & 0.2549 & 0.6471 \\ \hline
% lf\_bind & 3 & 1 & 0.1095 & 0.0871 & 0.0765 & 104 & 72 & 0.5909 & 0.6989 \\ \hline
% lf\_interact & 4 & 1 & 0.0274 & 0.0212 & 0.0180 & 23 & 21 & 0.5227 & 0.6591 \\ \hline
% lf\_affinity & 5 & 1 & 0.0523 & 0.0367 & 0.0292 & 63 & 21 & 0.75 & 0.5595 \\ \hline
% lf\_activate & 6 & 2 & 0.1195 & 0.0946 & 0.0790 & 66 & 126 & 0.3438 & 0.6615 \\ \hline
% lf\_increase & 7 & 2 & 0.1077 & 0.0821 & 0.0703 & 82 & 91 & 0.4740 & 0.6532 \\ \hline
% lf\_induce & 8 & 2 & 0.1512 & 0.1294 & 0.1145 & 68 & 175 & 0.2798 & 0.7572 \\ \hline
% lf\_stimulate & 9 & 2 & 0.0380 & 0.0317 & 0.0268 & 18 & 43 & 0.2951 & 0.7049 \\ \hline
% lf\_upregulate & 10 & 2 & 0.0100 & 0.0081 & 0.0068 & 5 & 11 & 0.3125 & 0.6875 \\ \hline
% lf\_downregulate & 11 & 3 & 0.0205 & 0.0193 & 0.0174 & 23 & 10 & 0.6970 & 0.8485 \\ \hline
% lf\_reduce & 12 & 3 & 0.0616 & 0.0535 & 0.0429 & 56 & 43 & 0.5657 & 0.6970 \\ \hline
% lf\_inhibit & 13 & 3 & 0.3230 & 0.1973 & 0.1842 & 358 & 161 & 0.6898 & 0.5703 \\ \hline
% lf\_decrease & 14 & 3 & 0.0585 & 0.0492 & 0.0473 & 50 & 44 & 0.5319 & 0.8085 \\ \hline
% lf\_agonist & 15 & 4 & 0.0535 & 0.0429 & 0.0429 & 44 & 42 & 0.5116 & 0.8023 \\ \hline
% lf\_antagonist & 16 & 5 & 0.0803 & 0.0572 & 0.0572 & 75 & 54 & 0.5814 & 0.7132 \\ \hline
% lf\_modulate & 17 & 6 & 0.0236 & 0.0156 & 0.0156 & 1 & 37 & 0.0263 & 0.6579 \\ \hline
% lf\_allosteric & 18 & 6 & 0.0081 & 0.0081 & 0.0081 & 6 & 7 & 0.4615 & 1 \\ \hline
% lf\_cofactor & 19 & 7 & 0.0050 & 0.0037 & 0.0037 & 5 & 3 & 0.625 & 0.75 \\ \hline
% lf\_substrate & 20 & 8 & 0.0230 & 0.0168 & 0.0137 & 22 & 15 & 0.5946 & 0.5946 \\ \hline
% lf\_transport & 21 & 8 & 0.0436 & 0.0324 & 0.0286 & 29 & 41 & 0.4143 & 0.6571 \\ \hline
% lf\_catalyze & 22 & 8 & 0.0274 & 0.0143 & 0.0106 & 32 & 12 & 0.7273 & 0.3864 \\ \hline
% lf\_product & 23 & 8 & 0.0585 & 0.0436 & 0.0429 & 19 & 75 & 0.2021 & 0.7340 \\ \hline
% lf\_convert & 24 & 8 & 0.0137 & 0.0106 & 0.0068 & 12 & 10 & 0.5455 & 0.5 \\ \hline
% \end{tabular}
% \caption{Previous Accuracy for Each Label Function}
% \end{table}



% \newpage
% \begin{table}[t!]
% \caption{Test accuracy (ChemPort,  Massive)/F1 scores (Claude9) of supervised-only methods and CFT across different proportions of clean data used,  label models,  and datasets. 
% % {\sc n/a} denotes an incompatibility between a method,  feature representation,  and/or task---see Appendix. 
% \textbf{First} and \underline{second} best results are \textbf{Bolded} and \underline{underlined}. \\ 
% %\todo{New results will be put into the table}
% }
% \label{tab:sweep label model}
% \begin{center}
% \begin{small}
% \begin{sc}
% % \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{lcccccccc}
% \toprule
%               & Claude9 &  ChemProt\tablefootnote{This is the ChemProt with updated LFs} & Massive &  \\
            
% \midrule
% \textbf{6.25\% Validation Size} &  &  &  \\
%     +Majority vote   & \underline{0.1532$\pm$0.0256}  & \textbf{0.6246$\pm$0.0181}  & \textbf{0.8110$\pm$0.0042}  \\
%     +DawidSkene     & \textbf{0.1533$\pm$0.0251}  & 0.6100$\pm$0.0199  & 0.7968$\pm$0.0103   \\
%     +Snorkel          & 0.1322$\pm$0.0217  & \underline{0.6168$\pm$0.0116}  & \underline{0.8106$\pm$0.0074} \\
%     +FlyingSquid      & 0.1090$\pm$0.0046  & 0.6058$\pm$0.0209  & 0.7507$\pm$0.0109   \\
%     +Supervised Only  & 0.1093$\pm$0.0048  & 0.5037$\pm$0.0296  & 0.7531$\pm$0.0136   \\
% \midrule
% \textbf{12.5\% Validation Size} &  &  &  \\
%     +Majority vote   & \underline{0.1747$\pm$0.0198}  & \textbf{0.6850$\pm$0.0104}  & \underline{0.8448$\pm$0.0060} \\
%     +DawidSkene       & \textbf{0.1840$\pm$0.0220}  & \underline{0.6540$\pm$0.0244}  & 0.8357$\pm$0.0038  \\
%     +Snorkel          & 0.1565$\pm$0.0159  & 0.6485$\pm$0.0147  & \textbf{0.8451$\pm$0.0048 }  \\
%     +FlyingSquid      & 0.1239$\pm$0.0143  & 0.6395$\pm$0.0152  & 0.8181$\pm$0.0092   \\
%     +Supervised Only & 0.1232$\pm$0.0150  & 0.5854$\pm$0.0219  & 0.8203$\pm$0.0128 \\
% \midrule
% \textbf{25\% Validation Size} &  &  &  \\
%     +Majority vote   & \underline{0.3448$\pm$0.1136}  & \textbf{0.7263$\pm$0.0210 } & \underline{0.8625$\pm$0.0040}   \\
%     +DawidSkene       & \textbf{0.3623$\pm$0.1074}  & \underline{0.7119$\pm$0.0136}  & \textbf{0.8626$\pm$0.0070} \\
%     +Snorkel          & 0.3028$\pm$0.0898  & 0.7114$\pm$0.0165  & 0.8585$\pm$0.0021   \\
%     +FlyingSquid     & 0.1700$\pm$0.0248  & 0.6957$\pm$0.0101  & 0.8563$\pm$0.0086   \\
%     +Supervised Only  & 0.1653$\pm$0.0521  & 0.6836$\pm$0.0234  & 0.8545$\pm$0.0095   \\
% \midrule
% \textbf{50\% Validation Size} &  &  &  \\
%     +Majority vote   & \textbf{0.4830$\pm$0.0714}  & \textbf{0.7783$\pm$0.0052} & 0.8824$\pm$0.0052   \\
%     +DawidSkene       & \underline{0.4769$\pm$0.0744}  & \underline{0.7749$\pm$0.0027}  & \underline{0.8843$\pm$0.0047} \\
%     +Snorkel          & 0.4624$\pm$0.0649  & 0.7669$\pm$0.0090  & \textbf{0.8853$\pm$0.0054 } \\
%     +FlyingSquid      & 0.2319$\pm$0.0565  & 0.7618$\pm$0.0075  & 0.8795$\pm$0.0049   \\
%     +Supervised Only  & 0.2531$\pm$0.0429  & 0.7731$\pm$0.0099  & 0.8825$\pm$0.0042   \\
% \midrule
% \textbf{100\% Validation Size} &  &  &  \\
%     +Majority vote    & \textbf{0.5819$\pm$0.0357} & \textbf{0.8199$\pm$0.0041 } & \textbf{0.8993$\pm$0.0021}  \\
%     +DawidSkene       & \underline{0.5724$\pm$0.0377}  & \underline{0.8197$\pm$0.0050}  & 0.8932$\pm$0.0019  \\
%     +Snorkel         & 0.5573$\pm$0.0195  & 0.8143$\pm$0.0041  & \underline{0.8988$\pm$0.0023}  \\
%     +FlyingSquid      & 0.3521$\pm$0.0374  & 0.8133$\pm$0.0060  & 0.8943$\pm$0.0050   \\
%     +Supervised Only  & 0.3473$\pm$0.0201  & 0.8162$\pm$0.0065  & 0.8975$\pm$0.0029   \\

% \bottomrule
% \end{tabular}
% % }
% \end{sc}
% \end{small}
% \end{center}
% \end{table}


